On the Randomized Complexity of Minimizing a Convex Quadratic Function

Minimizing a convex, quadratic objective of the form $f_{\mathbf{A},\mathbf{b}}(x) := \frac{1}{2}x^\top \mathbf{A} x - \langle \mathbf{b}, x \rangle$ for $\mathbf{A} \succ 0 $ is a fundamental problem in machine learning and optimization. In this work, we prove gradient-query complexity lower bounds for minimizing convex quadratic functions which apply to both deterministic and \emph{randomized} algorithms. Specifically, for $\kappa > 1$, we exhibit a distribution over $(\mathbf{A},\mathbf{b})$ with condition number $\mathrm{cond}(\mathbf{A}) \le \kappa$, such that any \emph{randomized} algorithm requires $\Omega(\sqrt{\kappa})$ gradient queries to find a solution $\hat x$ for which $\|\hat x - \mathbf x_\star\| \le \epsilon_0\|\mathbf{x}_{\star}\|$, where $\mathbf x_{\star} = \mathbf{A}^{-1}\mathbf{b}$ is the optimal solution, and $\epsilon_0$ a small constant. Setting $\kappa =1/\epsilon$, this lower bound implies the minimax rate of $T = \Omega(\lambda_1(\mathbf{A})\|\mathbf x_\star\|^2/\sqrt{\epsilon})$ queries required to minimize an arbitrary convex quadratic function up to error $f(\hat{x}) - f(\mathbf x_\star) \le \epsilon$. Our lower bound holds for a distribution derived from classical ensembles in random matrix theory, and relies on a careful reduction from adaptively estimating a planted vector $\mathbf u$ in a deformed Wigner model. A key step in deriving sharp lower bounds is demonstrating that the optimization error $\mathbf x_\star - \hat x$ cannot align too closely with $\mathbf{u}$. To this end, we prove an upper bound on the cosine between $\mathbf x_\star - \hat x$ and $\mathbf u$ in terms of the MMSE of estimating the plant $\mathbf u$ in a deformed Wigner model. We then bound the MMSE by carefully modifying a result due to Lelarge and Miolane 2016, which rigorously establishes a general replica-symmetric formula for planted matrix models.

==> into_spike.tex <==
%!TEX root = main_quad_lb.tex

\subsection{Lower Bound for Estimation of $\matu$\label{sec:matu_estimation}}

Having reduced the problem to estimating $\matu$, we conclude by bounding on the number of queries required to ensure that $\frac{\xhat}{\|\xhat\|} \in \sphered$ has a sufficiently large inner product with the planted solution $\matu$. 
%
To do so, we observe that an RQA interacting with an instance $(\matA,\matb)$ is equivalent to interacting with an instance $(\matM,\matb)$, since $\matA = (2(\lambda + \lambda^{-1}) - 2) I - \matM$. Moreover, without loss of generality we can bound
\begin{align*}
\langle \frac{\xhat}{\|\xhat\|},\matu \rangle^2 \le \| \Proj_{\vone,\dots,\vTplus}\matu\|_2^2,
\end{align*}
since we can assume without loss of generality that the $\itT+1$-st query made by our algorithm $\Alg$ to be $\vTplus = \xhat$.
%
With this reduction in place, we have the following theorem:

\begin{thm}\label{thm:est_u_lb} Let $\lambda \in (1,\frac{3}{2}]$ and $\taub = (\lambda - 1)^2$, and let $\matu$, $\matM$ and $\matb$ be as in Section~\ref{sec:reduction}. Then for any RQA $\Alg$ interacting with the instances $(\matM,\matb)$,
\begin{align*}
\Pr_{\matu,\matM,\matb,\Alg}\left[ \langle \uhat, \matu \rangle^2 >   2 e \cdot \tau_0 \itT  \right] \nonumber  \le \deltaexp
\end{align*}
where the probability is taken over the randomness of the algorithm, and over $\matu,\matb,\matW$. 
\end{thm}
For intuition, we recall that $\taub$ controls the initial information about $\matu$ conveyed by $\matb$, via $\Exp\langle \bnot, \matu \rangle^2 = \taub + o(1)$. Moreover, $\| \Proj_{\vone,\dots,\vTplus}\matu\|_2^2$ controls the amount of information about $\matu$ acquired by the queries $\vone,\dots,\vTplus$. 
%
Hence, Theorem~\ref{thm:est_u_lb} says that the rate of information acquired grows as the first $\BigOh{\itT}$ terms of a geometric series with base $\lambda^{\BigOh{1}}$, multiplied by the initial information $\taub$.
%
In particular, if $c_1$ is the constant from Proposition~\ref{prop:minimax_red} (or Propostion~\ref{prop:not_minimax_red}), and if $\itT \le \frac{1 \wedge c_1}{16(\lambda - 1)}$, we have that
\begin{align*}
2\lambda^{4\itT+2} \cdot \taub\sum_{j=1}^{\itT} \lambda^{4j} \le 2 \taub \itT \lambda^{8\itT+2} \le \frac{\taub\lambda^{5/2}}{8c_1(\lambda - 1)} \le \frac{\taub}{c_1(\lambda - 1)}~.
\end{align*}
Hence, by Theorem~\ref{thm:est_u_lb} and absorbing constants into the $\dellam$, we have that for $\itT \le \frac{1 \wedge c_1}{16(\lambda - 1)}$~,
\begin{align}\label{eq:lb_conseq}
\Pr_{\matu,\matM,\matb,\Alg}\left[\|\Proj_{\vone,\dots,\vTplus}\matu\|_2^2 >  \frac{\taub}{c_1(\lambda - 1)} \right] \le 
\frac{e^{ -d  \lambda^2\taub (\lambda - 1)/5}}{16^2(\lambda - 1)^2}  + 2e^{-\tfrac{d^{1/4}}{8}} \le \dellam~.
\end{align}

T


\iffalse
\begin{cor} In the settings of Theorem~\ref{thm:reduction_to_main} and~\ref{thm:est_u_lb}, we have that for any algorith with query complexity at most $\itT$
\begin{eqnarray}
 \Pr\left[\Eerr(\mult,t) \big{|} \left\{\cond(\matA) \le \mult \cdot \conddet(\lambda)\right\} \cap \Eovlap(t)\right] \le \deltaexp
\end{eqnarray}
Hence, for any fixed constant $t > 1$ (say $ t= 2$), there exists a distribution over instances $(\matA,\matb)$ for which $\Pr_{\matA,\matb,\Alg}[\left\{\frac{\|\matxst - \xhat\|_2}{\|\matxst\|_2} \le \frac{\taub }{4\mult t(\lambda -1)\cdot\ovlapd} \right\}]$ for any $\Alg$ with ...
\end{cor}
\fi







==> organization.tex <==
%!TEX root = main_quad_lb.tex

\subsection{Organization}

==> overlap_sec.tex <==
%!TEX root = main_quad_lb.tex

\iffalse
\begin{conj}[Non-Asymptotic Convergence]\label{conj:nonasymp} There exists universal constants $c_1,c_2,c_3, d_0 > 0$ such that, for all $\mu \in []$ and $\lambda > 1$ and $d \ge d_0$ then defining the sequence of distributions  $\matM \sim []$ and $\matu$, \emph{either} (a)
\begin{align*}
\MMSE(\matutil;\matMtil) \ge \lim_{d \to \infty} \MMSE(\matutil;\matMtil) - d^{-c_1}(\lambda - 1)^{c_2} ()^{c_3}
\end{align*}
or (b)
\begin{align*}
|\info(\matW + \lambda \matutil \matutil^{\top};\matutil \matutil^{\top}) - \lim_{d \to \infty} \info(\matW + \lambda \matutil \matutil^{\top};\matutil \matutil^{\top})| \le d^{-c_1}(\lambda - 1)^{c_2} ()^{c_3}
\end{align*}
\end{conj}

\begin{prop}Conjecture~\ref{conj:nonasymp} part (b) implies Conjecture~\ref{conj:nonasymp} part (a), and Conjecture~\ref{conj:nonasymp} part (a) implies that, if $\dots$, then
\begin{align*}
\ovlapd(\taub) \le 
\end{align*}
\end{prop}

It thus natural to define the follow auxillary overlap function,


 Next by working out the general formula of Lelarge and Miolane, we can compute that


Moreover, a standard Gaussian concentration argument shows that, if we define $\boldalpha := \|\bnot,\sqrt{(1+\taub)}\|$



In particular, at $\lambda = 1$, the top eigenvector of $\matM$ has vanishing overlap with $\matu$. This value $\lambda = 1$ is known as the 'information-theoretic threshold', and because for any $0 \le \lambda \le $,  the distributions of the deformed Wigner $\matM = \matW + \lambda \matu \matu^\top$ and the standard Wigner ensemble $\matW$ become information-theoretically indistinguishable[cite]. 

On the other hand, when $\lambda > 1$, a simple 

 we are operating near the ``information-theoretic threshold''




\begin{defn}[Overlap Function] 
\begin{eqnarray}
\ovlapd(\mu,\lambda)^2 &:=& \Exp[\|\matutil\|_2^2]^2 -  \Exp_{\matutil}\Exp_{\matMtil}\left[ \|\matutil \matutil^\top -  \Exp[\matutil\matutil^{\top} | \matMtil] \|_{\F}^2 \big{|}\matutil \right]~,
\end{eqnarray}
where $\matutil_i \overset{(i.i.d)}{\sim} \mathcal{N}(\mu/\sqrt{d},1/d)$, and $\matMtil := \matW + \lambda \matutil\matutil^\top$. 
\end{defn}
Note that 



\begin{thm}[Specialization of Lelarge]\label{thm:lelarge}
\begin{eqnarray}
\ovlapst(\mu,\lambda) := \lim_{d \to \infty} \ovlapd(\mu,\lambda) \le \mu^2 + 1 - \frac{1}{\lambda^2} + \frac{|\mu|}{\lambda}~.
\end{eqnarray}
%where $X_0 \sim \mathcal{N}(\mu,\sigma^2)$, and 
\end{thm}

\begin{lem}\label{lem:ovlap_conversion}
For any $\uhat \in \sphered$ such that  $\uhat \perp (\matM,\bnot) \big{|} \matu$, and define 

Then, $\ovlapdbar(\tau) := \max_{\alpha: |\alpha - 1| \le d^{-1/4}} \frac{\ovlapd(\sqrt{\tau}\alpha,\lambda/(1+\tau))}{1+\tau}$~.
\end{lem}
\fi


==> proof_of_main.tex <==
%!TEX root = main_quad_lb.tex
\subsection{Proof of Main Results\label{sec:main_result_proof}}
\begin{proof}[Proof of Theorem~\ref{thm:main_theorem}]

Fix $\condnum \ge 40$, and let $\taub = (\lambda - 1)^2$, and let $\lambda = 1 + \sqrt{\frac{10}{\condnum}}$; note that $\lambda \in (1,\tfrac{3}{2}]$. Moreover, let $\matAtil,\matbtil,\matxsttil$ be as in Proposition~\ref{prop:minimax_red}.
By Propostion~\ref{prop:minimax_red}, we have that with probability $1$, 
	\begin{align*}
	\conddet(\matAtil) \le 2\conddet(\lambda) := 2 \cdot \frac{2(\lambda^2 + 1)}{(\lambda - 1)^2}  \le 10/(\lambda - 1)^2 \text{ for } \lambda \in (1,\frac{3}{2}].
\end{align*}
Now, let $c_1,c_2$ be the constants  in Propostion~\ref{prop:minimax_red}. Then, for imply that for $\itT \le \frac{1 \wedge c_1}{16(\lambda - 1)}$ we have that by Propostion~\ref{prop:minimax_red} and Theorem~\ref{thm:est_u_lb},
\begin{align*}
	\frac{1}{4}\Pr_{\matAtil,\matbtil \sim \calD}\Pr_{\Alg}\left[ \frac{\|\xhat - \matxsttil\|_2^2}{\|\matxsttil\|_2^2 } \le \frac{c_2}{K} \right]  \le \dellam + \dellam = \dellam.
\end{align*}
By Propostion~\ref{prop:ovlap_prop}, the function $d_1 = d_1(\lambda) = d_1(\condnum)$ is such that for any $d \ge d_1(\condnum)$, we can take $K = 5$ in the above bound. Hence, 
\begin{align*}
	\Pr_{\matAtil,\matbtil \sim \calD}\Pr_{\Alg}\left[ \frac{\|\xhat - \matxsttil\|_2^2}{\|\matxsttil\|_2^2 } \le \frac{c_2}{5} \right]  \le 4 \dellam = \dellam.
\end{align*}
 Note that under Conjecture~\ref{conj:nonasymp}, Proposition~\ref{prop:ovlap_prop} implies that $d_1(\lambda) = \BigOh{\poly(\lambda - 1)^{-1}}$, which by our choice of $\condnum$ implies that we can write $d_1 = d_1(\condnum) = \BigOh{\poly(\condnum) } $. Moreover, we have
	\begin{align*}
	f_{\matAtil,\matbtil}(\xhat) - f_{\matAtil,\matbtil}(\matxsttil)~\ge~ \lambda_{d}(\matAtil)\|\xhat - \matxsttil\|_2^2~=~ \frac{\lambda_1(\matAtil)}{\cond(\matA)}\|\xhat - \matxsttil\|_2^2 ~\ge~ \frac{\lambda_1(\matAtil)}{\condnum}\|\xhat - \matxsttil\|_2^2~,
	\end{align*}
	which implies that
	\begin{align*}
	&\Pr_{\matAtil,\matbtil \sim \calD}\Pr_{\Alg}\left[ \left\{\|\xhat - \matxsttil\|_2^2 \le \frac{c_2}{5} \|\matxsttil\|_2^2\right\} \vee \left\{f_{\matAtil,\matbtil}(\xhat) - f_{\matAtil,\matbtil}(\matxsttil) \le  \frac{c_2}{5} \frac{\lambda_1(\matAtil)\|\matxsttil\|_2^2}{\condnum} \right\} \right] \\
	&= \Pr_{\matAtil,\matbtil \sim \calD}\Pr_{\Alg}\left[ \|\xhat - \matxsttil\|_2^2 \ge \frac{c_2}{5} \|\matxsttil\|_2^2 \right] \le  \dellam.
	\end{align*}
	Finally, we reparameterize $c_1' \leftarrow \frac{1 \wedge c_1}{16\cdot 10}$, and $c_2' \leftarrow c_2/5$, and observe by definition of $\dellam$, there is a $d_0(\condnum) = \BigOh{\poly(\condnum)}$ such that for $d \ge d_0(\condnum)$, $\dellam = e^{-c_3d^{-c_4}}$ for universal constants $c_3,c_4 > 0$. With these new constants, we have shown that for $\itT \le c_1'/\sqrt{\kappa} = \frac{1 \wedge c_1}{16 (\lambda -1)}$, we have
	\begin{align*}
	&\Pr_{\matAtil,\matbtil \sim \calD}\Pr_{\Alg}\left[ \left\{\|\xhat - \matxsttil\|_2^2 \le c_2' \|\matxsttil\|_2^2\right\} \vee \left\{f_{\matAtil,\matbtil}(\xhat) - f_{\matAtil,\matbtil}(\matxsttil) \le c_2'\frac{\lambda_1(\matAtil)\|\matxsttil\|_2^2}{\condnum} \right\} \right] \le  e^{-c_3d^{-c_4}},
	\end{align*}
	as needed.

\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:polynomial_theorem}]
The proof of Theorem~\ref{thm:polynomial_theorem} is almost identical to that of Theorem~\ref{rem:main_thm}. The only differences are that (a) we use Proposition~\ref{prop:not_minimax_red}, which translates into an upper bound bound on the event $\{\frac{\|\xhat - \matxsttil\|_2^2}{\|\matxsttil\|_2^2 } \lesssim \frac{1}{\lambda - 1}\} = \{\frac{\|\xhat - \matxsttil\|_2^2}{\|\matxsttil\|_2^2 } \lesssim \frac{1}{\sqrt{\condnum}}\} $, (b) we use the original distribution $(\matA,\matb)$ rather than the conditioned-distribution $(\matAtil,\matbtil)$, (c) because of not conditioning, we have the guarantee $\Pr[\cond(\matA) \le \condnum] \ge 1 - e^{-c_3d^{-c_4}}$ (but not with probability $1$), and (d) because we don't need Proposition~\ref{prop:ovlap_prop}, there is no need to ensure $d \ge d_1(\condnum)$.
\end{proof}
